Deep Permutation Equivariant Structure from Motion

Existing deep methods produce highly accurate 3D reconstructions in stereo and multiview stereo settings, i.e., when cameras are both internally and externally calibrated. Nevertheless, the challenge of simultaneous recovery of camera poses and 3D scene structure in multiview settings with deep networks is still outstanding. Inspired by projective factorization for Structure from Motion (SFM) and by deep matrix completion techniques, we propose a neural network architecture that, given a set of point tracks in multiple images of a static scene, recovers both the camera parameters and a (sparse) scene structure by minimizing an unsupervised reprojection loss. Our network architecture is designed to respect the structure of the problem: the sought output is equivariant to permutations of both cameras and scene points. Notably, our method does not require initialization of camera parameters or 3D point locations. We test our architecture in two setups: (1) single scene reconstruction and (2) learning from multiple scenes. Our experiments, conducted on a variety of datasets in both internally calibrated and uncalibrated settings, indicate that our method accurately recovers pose and structure, on par with classical state of the art methods. Additionally, we show that a pre-trained network can be used to reconstruct novel scenes using inexpensive fine-tuning with no loss of accuracy.

==> LaTeX/tables/calibrated_exp.tex <==
\begin{table*}[tb]
    \hspace{-8pt}
    \setlength\tabcolsep{1pt} % default value: 6pt
    \tiny
    \centering
    \begin{tabular}{c}
        \begin{adjustbox}{max width=\textwidth}
        \aboverulesep=0ex
        \belowrulesep=0ex
        \renewcommand{\arraystretch}{0.9}
        \begin{tabular}[t]{|l|r|r||rrrr|rrrr|rrrr|}
            \hline
            \multirow{2}{3em}{Scan}& \multirow{2}{3em}{\#Images} & \multirow{2}{3em}{\#Points} & \multicolumn{4}{c|}{$\tr_{\text{error}}$} & \multicolumn{4}{c|}{$R_{\text{error}}$} & \multicolumn{4}{c|}{Reprojection Error} \\
            & & &  \textbf{Ours} & GESFM & Linear & Colmap & \textbf{Ours} & GESFM & Linear & Colmap & \textbf{Ours} & GESFM & Linear & Colmap  \\
			\hline
Alcatraz Courtyard & $ 133 $ & $ 23674 $ & $ 0.015 $ & $ 0.259 $ & $\mathbf{0.014}$ & $\mathbf{0.014}$ & $ 0.049 $ & $ 0.533 $ & $\mathbf{0.042}$ & $ 0.043 $ & $\mathbf{0.81}$ & $ 4.67 $ & $ 1.27 $ & $\mathbf{0.81}$\\
Alcatraz Water Tower & $ 172 $ & $ 14828 $ & $ 0.116 $ & $ 9.147 $ & $ 1.643 $ & $\mathbf{0.115}$ & $ 0.23 $ & $ 9.997 $ & $ 1.525 $ & $\mathbf{0.228}$ & $\mathbf{0.55}$ & $ 25.93 $ & $ 73.72 $ & $\mathbf{0.55}$\\
Buddah Tooth Relic Temple Singapore & $ 162 $ & $ 27920 $ & $\mathbf{0.014}$ & $ 1.429 $ & $ 0.125 $ & $ 0.015 $ & $\mathbf{0.081}$ & $ 4.709 $ & $ 0.551 $ & $ 0.083 $ & $\mathbf{0.85}$ & $ 13.22 $ & $ 2.66 $ & $\mathbf{0.85}$\\
Doge Palace Venice & $ 241 $ & $ 67107 $ & $ 0.029 $ & $ 1.608 $ & - & $\mathbf{0.012}$ & $ 0.211 $ & $ 5.317 $ & - & $\mathbf{0.031}$ & $ 1.0 $ & $ 22.32 $ & - & $\mathbf{0.98}$\\
Door Lund & $ 12 $ & $ 17650 $ & $\mathbf{0.001}$ & $ (0.973) $ & $\mathbf{0.001}$ & $\mathbf{0.001}$ & $ 0.006 $ & $ (7.552) $ & $\mathbf{0.005}$ & $\mathbf{0.005}$ & $\mathbf{0.3}$ & $ (9.21) $ & $\mathbf{0.3}$ & $\mathbf{0.3}$\\
Drinking Fountain Somewhere In Zurich & $ 14 $ & $ 5302 $ & $\mathbf{0.002}$ & $ (0.002) $ & $\mathbf{0.002}$ & $\mathbf{0.002}$ & $\mathbf{0.007}$ & $ (0.01) $ & $\mathbf{0.007}$ & $\mathbf{0.007}$ & $ 0.31 $ & $ (0.27) $ & $ 0.31 $ & $ 0.31 $\\
East Indiaman Goteborg & $ 179 $ & $ 25655 $ & $ 0.509 $ & $ 3.099 $ & $ (2.235) $ & $\mathbf{0.065}$ & $ 3.117 $ & $ 12.396 $ & $ (3.284) $ & $\mathbf{0.251}$ & $ 1.85 $ & $ 32.37 $ & $ (312.9) $ & $\mathbf{0.89}$\\
Ecole Superior De Guerre & $ 35 $ & $ 13477 $ & $ 0.005 $ & $ (0.002) $ & $ 0.005 $ & $ 0.005 $ & $\mathbf{0.024}$ & $ (0.035) $ & $\mathbf{0.024}$ & $\mathbf{0.024}$ & $ 0.34 $ & $ (0.14) $ & $ 0.34 $ & $ 0.34 $\\
Eglise du dome & $ 85 $ & $ 84792 $ & $\mathbf{0.01}$ & $ (1.425) $ & $ 0.046 $ & $\mathbf{0.01}$ & $ 0.037 $ & $ (3.631) $ & $ 0.162 $ & $\mathbf{0.036}$ & $\mathbf{0.27}$ & $ (6.21) $ & $ 0.76 $ & $\mathbf{0.27}$\\
Folke Filbyter & $ 40 $ & $ 21150 $ & $ 0.118 $ & $ (0.0) $ & $ 0.123 $ & $\mathbf{0.0}$ & $ 70.157 $ & $ (0.148) $ & $ 4.484 $ & $\mathbf{0.036}$ & $ 4.29 $ & $ (0.41) $ & $ 6.06 $ & $\mathbf{0.29}$\\
Fort Channing Gate Singapore & $ 27 $ & $ 23627 $ & $\mathbf{0.008}$ & $\mathbf{0.008}$ & $ 0.013 $ & $\mathbf{0.008}$ & $\mathbf{0.02}$ & $\mathbf{0.02}$ & $ 0.029 $ & $\mathbf{0.02}$ & $\mathbf{0.25}$ & $\mathbf{0.25}$ & $ 0.45 $ & $\mathbf{0.25}$\\
Golden Statue Somewhere In Hong Kong & $ 18 $ & $ 39989 $ & $\mathbf{0.004}$ & $\mathbf{0.004}$ & $\mathbf{0.004}$ & $\mathbf{0.004}$ & $ 0.031 $ & $ 0.03 $ & $\mathbf{0.022}$ & $ 0.031 $ & $\mathbf{0.27}$ & $\mathbf{0.27}$ & $ 0.3 $ & $\mathbf{0.27}$\\
Gustav Vasa & $ 18 $ & $ 4249 $ & $ 1.145 $ & $ (0.101) $ & $\mathbf{0.099}$ & $ 0.1 $ & $ 32.266 $ & $ (0.751) $ & $ 0.839 $ & $ 0.841 $ & $ 3.15 $ & $ (0.31) $ & $ 0.48 $ & $ 0.48 $\\
GustavIIAdolf & $ 57 $ & $ 5813 $ & $ 8.524 $ & $\mathbf{0.004}$ & $\mathbf{0.004}$ & $\mathbf{0.004}$ & $ 58.458 $ & $\mathbf{0.021}$ & $\mathbf{0.021}$ & $\mathbf{0.021}$ & $ 11.49 $ & $\mathbf{0.26}$ & $\mathbf{0.26}$ & $\mathbf{0.26}$\\
Jonas Ahlstromer & $ 40 $ & $ 2021 $ & $ 10.451 $ & $ (0.01) $ & $ 1.259 $ & $ 0.011 $ & $ 47.117 $ & $ (0.082) $ & $ 5.391 $ & $\mathbf{0.036}$ & $ 8.41 $ & $ (0.69) $ & $ 4.69 $ & $\mathbf{0.22}$\\
King's College University Of Toronto & $ 77 $ & $ 7087 $ & $ 0.017 $ & $ (0.005) $ & $ (1.877) $ & $ 0.017 $ & $ 0.085 $ & $ (0.059) $ & $ (4.624) $ & $ 0.084 $ & $\mathbf{0.34}$ & $ (0.35) $ & $ (7.12) $ & $\mathbf{0.34}$\\
Lund University Sphinx & $ 70 $ & $ 32668 $ & $ 2.191 $ & $ 0.016 $ & $ 1.512 $ & $\mathbf{0.009}$ & $ 8.752 $ & $ 0.058 $ & $ 5.452 $ & $\mathbf{0.033}$ & $ 1.36 $ & $ 0.4 $ & $ 4.58 $ & $\mathbf{0.39}$\\
Nijo Castle Gate & $ 19 $ & $ 7348 $ & $ 0.012 $ & $\mathbf{0.011}$ & $ 0.19 $ & $\mathbf{0.011}$ & $ 0.069 $ & $\mathbf{0.064}$ & $ 0.744 $ & $\mathbf{0.064}$ & $\mathbf{0.73}$ & $\mathbf{0.73}$ & $ 4.84 $ & $\mathbf{0.73}$\\
Pantheon Paris & $ 179 $ & $ 29383 $ & $\mathbf{0.005}$ & $ 0.595 $ & $ 0.011 $ & - & $\mathbf{0.04}$ & $ 3.208 $ & $ 0.072 $ & - & $\mathbf{0.49}$ & $ 9.71 $ & $ 0.82 $ & -\\
Park Gate Clermont Ferrand & $ 34 $ & $ 9099 $ & $\mathbf{0.022}$ & $\mathbf{0.022}$ & $\mathbf{0.022}$ & $\mathbf{0.022}$ & $\mathbf{0.049}$ & $\mathbf{0.049}$ & $\mathbf{0.049}$ & $\mathbf{0.049}$ & $\mathbf{0.35}$ & $\mathbf{0.35}$ & $\mathbf{0.35}$ & $\mathbf{0.35}$\\
Plaza De Armas Santiago & $ 240 $ & $ 26969 $ & $ 1.383 $ & $ 2.244 $ & - & $\mathbf{0.048}$ & $ 2.556 $ & $ 6.344 $ & - & $\mathbf{0.122}$ & $ 4.9 $ & $ 15.61 $ & - & $\mathbf{1.13}$\\
Porta San Donato Bologna & $ 141 $ & $ 25490 $ & $\mathbf{0.046}$ & $ 0.169 $ & $ 0.067 $ & $ 0.047 $ & $\mathbf{0.095}$ & $ 0.513 $ & $ 0.149 $ & $ 0.099 $ & $\mathbf{0.75}$ & $ 3.23 $ & $ 1.16 $ & $\mathbf{0.75}$\\
Round Church Cambridge & $ 92 $ & $ 84643 $ & $ 0.582 $ & $ 0.493 $ & $\mathbf{0.012}$ & $\mathbf{0.012}$ & $ 1.107 $ & $ 1.851 $ & $\mathbf{0.033}$ & $ 0.035 $ & $ 1.54 $ & $ 2.03 $ & $ 0.41 $ & $\mathbf{0.39}$\\
Skansen Kronan Gothenburg & $ 131 $ & $ 28371 $ & $ 0.008 $ & $ 0.008 $ & $ (0.007) $ & $ 0.008 $ & $ 0.026 $ & $ 0.025 $ & $ (0.02) $ & $ 0.025 $ & $\mathbf{0.67}$ & $\mathbf{0.67}$ & $ (0.69) $ & $\mathbf{0.67}$\\
Smolny Cathedral St Petersburg & $ 131 $ & $ 51115 $ & $\mathbf{0.006}$ & $ 0.007 $ & - & $\mathbf{0.006}$ & $ 0.033 $ & $\mathbf{0.028}$ & - & $ 0.029 $ & $\mathbf{0.81}$ & $ 1.0 $ & - & $\mathbf{0.81}$\\
Some Cathedral In Barcelona & $ 177 $ & $ 30367 $ & $ 0.011 $ & $ 0.013 $ & $ 0.024 $ & $\mathbf{0.01}$ & $ 0.026 $ & $ 0.031 $ & $ 0.057 $ & $\mathbf{0.025}$ & $\mathbf{0.89}$ & $ 1.09 $ & $ 2.09 $ & $\mathbf{0.89}$\\
Sri Mariamman Singapore & $ 222 $ & $ 56220 $ & $\mathbf{0.023}$ & $ 0.614 $ & $ 0.025 $ & $\mathbf{0.023}$ & $\mathbf{0.077}$ & $ 2.158 $ & $ 0.083 $ & $ 0.078 $ & $ 0.91 $ & $ 7.4 $ & $ 1.17 $ & $\mathbf{0.89}$\\
Sri Thendayuthapani Singapore & $ 98 $ & $ 88849 $ & $ 2.87 $ & $ (0.053) $ & $\mathbf{0.034}$ & $\mathbf{0.034}$ & $ 44.17 $ & $ (0.329) $ & $\mathbf{0.138}$ & $\mathbf{0.138}$ & $ 8.44 $ & $ (0.56) $ & $ 0.72 $ & $ 0.67 $\\
Sri Veeramakaliamman Singapore & $ 157 $ & $ 130013 $ & $ 0.04 $ & $ (1.388) $ & $ 0.095 $ & $\mathbf{0.038}$ & $ 0.175 $ & $ (3.41) $ & $ 0.288 $ & $\mathbf{0.169}$ & $ 0.73 $ & $ (34.72) $ & $ 2.2 $ & $\mathbf{0.71}$\\
Statue Of Liberty & $ 134 $ & $ 49250 $ & $ 4.122 $ & $ (4.782) $ & $ 28.049 $ & $\mathbf{0.099}$ & $ 9.091 $ & $ (8.281) $ & $ 2.945 $ & $\mathbf{0.213}$ & $ 6.97 $ & $ (52.05) $ & $ 5.08 $ & $\mathbf{1.25}$\\
The Pumpkin & $ 196 $ & $ 69341 $ & $ 14.952 $ & $\mathbf{0.022}$ & $ (14.862) $ & $\mathbf{0.022}$ & $ 98.862 $ & $ 0.092 $ & $ (3.123) $ & $\mathbf{0.091}$ & $ 24.85 $ & $\mathbf{0.57}$ & $ (24.19) $ & $\mathbf{0.57}$\\
Thian Hook Keng Temple Singapore & $ 138 $ & $ 34288 $ & $\mathbf{0.008}$ & $ 0.024 $ & $ 0.043 $ & $\mathbf{0.008}$ & $\mathbf{0.081}$ & $ 0.245 $ & $ 0.424 $ & $ 0.084 $ & $ 1.13 $ & $ 3.32 $ & $ 4.92 $ & $\mathbf{1.12}$\\
Tsar Nikolai I & $ 98 $ & $ 37857 $ & $ 7.836 $ & $\mathbf{0.005}$ & $\mathbf{0.005}$ & $\mathbf{0.005}$ & $ 36.28 $ & $\mathbf{0.018}$ & $\mathbf{0.018}$ & $\mathbf{0.018}$ & $ 6.53 $ & $\mathbf{0.33}$ & $\mathbf{0.33}$ & $\mathbf{0.33}$\\
Urban II & $ 96 $ & $ 22284 $ & $ 9.586 $ & $ 0.036 $ & $ 3.038 $ & $\mathbf{0.021}$ & $ 48.214 $ & $ 0.175 $ & $ 16.348 $ & $\mathbf{0.107}$ & $ 6.92 $ & $ 0.72 $ & $ 17.61 $ & $\mathbf{0.38}$\\
Vercingetorix & $ 69 $ & $ 10754 $ & $ 3.104 $ & $ 0.3 $ & $ 1.564 $ & $\mathbf{0.011}$ & $ 17.706 $ & $ 1.431 $ & $ 7.138 $ & $\mathbf{0.048}$ & $ 1.5 $ & $ 0.54 $ & $ 2.93 $ & $\mathbf{0.23}$\\
Yueh Hai Ching Temple Singapore & $ 43 $ & $ 13774 $ & $\mathbf{0.014}$ & $ (0.023) $ & $ 0.059 $ & $\mathbf{0.014}$ & $\mathbf{0.043}$ & $ (0.075) $ & $ 0.26 $ & $\mathbf{0.043}$ & $\mathbf{0.65}$ & $ (1.64) $ & $ 2.06 $ & $\mathbf{0.65}$\\
    \bottomrule
	\end{tabular} 
	\end{adjustbox}
	\vspace{3pt}      
    \end{tabular}
    \caption{\small Single scene results with our method against baselines in the calibrated setup. The table shows mean camera location error (denoted $\tr_{\mathrm{error}}$) in meters, mean orientation error (denoted $R_{\mathrm{error}}$) in degrees, and mean reprojection error in pixels. (\textit{Smaller is better.}) In parenthesis experiments in which at least 10\% of the cameras are removed.}
    \label{tab:Euclidean_Results}
\end{table*}

==> LaTeX/tables/generalizing_times.tex <==
\begin{table*}[t]
    \hspace{-8pt}
    \setlength\tabcolsep{2pt} % default value: 6pt
    %\small
    \centering
    \scriptsize
    
    \begin{tabular}{c}
        \begin{adjustbox}{max width=\textwidth}
        \aboverulesep=0ex
        \belowrulesep=0ex
        \renewcommand{\arraystretch}{1}
        \begin{tabular}[t]{|l|r|r|rrrr|}
            \hline
            \multirow{2}{3em}{Scan}& \multirow{2}{3em}{\#Images} & \multirow{2}{3em}{\#Points} & \multicolumn{4}{c|}{\textbf{Time (seconds)}} \\
            \cline{4-7}
            & & & Inference & Fine tuning & BA & Colmap\\
            \hline
            Alcatraz Courtyard & 133 & 23674 & $ 0.007 $ & $ 199.125 $ & $ 43.512 $ & $ 286.0 $\\
Alcatraz Water Tower & 172 & 14828 & $ 0.007 $ & $ 110.847 $ & $ 26.44 $ & $ 130.0 $\\
Drinking Fountain Somewhere In Zurich & 14 & 5302 & $ 0.007 $ & $ 20.302 $ & $ 2.925 $ & $ 16.0 $\\
Nijo Castle Gate & 19 & 7348 & $ 0.008 $ & $ 24.493 $ & $ 4.308 $ & $ 21.0 $\\
Porta San Donato Bologna & 141 & 25490 & $ 0.007 $ & $ 194.651 $ & $ 45.416 $ & $ 170.0 $\\
Round Church Cambridge & 92 & 84643 & $ 0.014 $ & $ 360.97 $ & $ 90.092 $ & $ 229.0 $\\
Smolny Cathedral St Petersburg & 131 & 51115 & $ 0.004 $ & $ 534.528 $ & $ 101.456 $ & $ 516.0 $\\
Some Cathedral In Barcelona & 177 & 30367 & $ 0.007 $ & $ 208.542 $ & $ 55.424 $ & $ 451.0 $\\
Sri Veeramakaliamman Singapore & 157 & 130013 & $ 0.319 $ & $ 291.727 $ & $ 242.888 $ & $ 583.0 $\\
Yueh Hai Ching Temple Singapore & 43 & 13774 & $ 0.004 $ & $ 45.458 $ & $ 10.539 $ & $ 106.0 $\\
			\bottomrule
	\end{tabular} 
	
\begin{tabular}[t]{|l|r|r|rrrr|}
            \hline
            \multirow{2}{3em}{Scan}& \multirow{2}{3em}{\#Images} & \multirow{2}{3em}{\#Points} & \multicolumn{4}{c|}{\textbf{Time (seconds)}} \\
            \cline{4-7}
            & & & Inference & Fine tuning & BA & GPSFM\\
            \hline
Alcatraz Water Tower & 172 & 14828 & $ 0.055 $ & $ 89.646 $ & $ 68.939 $ & $ 137.057 $\\
Dino 319 & 36 & 319 & $ 0.004 $ & $ 8.151 $ & $ 0.475 $ & $ 3.253 $\\
Dino 4983 & 36 & 4983 & $ 0.122 $ & $ 7.66 $ & $ 2.21 $ & $ 4.994 $\\
Dome & 85 & 84792 & $ 0.203 $ & $ 160.896 $ & $ 76.867 $ & $ 105.837 $\\
Drinking Fountain & 14 & 5302 & $ 0.01 $ & $ 18.197 $ & $ 3.016 $ & $ 3.348 $\\
Gustav Vasa & 18 & 4249 & $ 0.007 $ & $ 14.435 $ & $ 2.766 $ & $ 3.449 $\\
Nijo & 19 & 7348 & $ 0.013 $ & $ 34.397 $ & $ 3.121 $ & $ 6.37 $\\
Skansen Kronan & 131 & 28371 & $ 0.141 $ & $ 197.531 $ & $ 63.853 $ & $ 93.831 $\\
Some Cathedral In Barcelona & 177 & 30367 & $ 0.133 $ & $ 185.984 $ & $ 47.597 $ & $ 110.485 $\\
Sri Veeramakaliamman Singapore & 157 & 130013 & $ 0.314 $ & $ 473.294 $ & $ 195.374 $ & $ 301.713 $\\
			\bottomrule
	\end{tabular} 
	
	\end{adjustbox}
	\vspace{3pt}      
    \end{tabular}
    \caption{\small Multiple scenes learning - calibrated (left) and uncalibrated (right) results times in seconds.
    }
    \label{tab:Generalizing_times}
\end{table*}

==> LaTeX/tables/models_ablation.tex <==
\begin{table*}[t]
\centering
    \hspace{-8pt}
    \setlength\tabcolsep{2pt} % default value: 6pt
    \scriptsize
    \begin{tabular}{c}
        \begin{adjustbox}{max width=\textwidth}
        \aboverulesep=0ex
        \belowrulesep=0ex
        \renewcommand{\arraystretch}{1}
        \begin{tabular}[t]{|l|rrr|}
            \hline
            \multirow{2}{3em}{Scan}& \multicolumn{3}{c|}{\textbf{Error (pixels)}}\\
            %\cline{4-8}
            & \textbf{Ours} & \textbf{Set Net.} & \textbf{Graph Net.} \\
			\hline
            \textbf{Geo. Mean Ratio} & $ 1.0 $ & $ 1.36 $ & $ 1.52 $\\
			\bottomrule
	\end{tabular} 
	\end{adjustbox}
	\vspace{3pt}      
    \end{tabular}
    \caption{\small Models comparison, }
    \label{tab:models_comparison}
\end{table*}

==> LaTeX/tables/projective_exp.tex <==
\begin{table}[tb]
    \hspace{-8pt}
    \setlength\tabcolsep{2pt} % default value: 6pt
    \tiny
    \centering
    \begin{tabular}{c}
        \begin{adjustbox}{max width=\textwidth}
        \aboverulesep=0ex
        \belowrulesep=0ex
        \renewcommand{\arraystretch}{1}
        \begin{tabular}[t]{|l|r|r|rrrr|}
            \hline
            \multirow{2}{3em}{Scan}& \multirow{2}{3em}{\#Images} & \multirow{2}{3em}{\#Points} & \multicolumn{4}{c|}{\textbf{Reprojection error (pixels)}}\\
            & & & \textbf{Ours} & GPSFM & PPSFM & VarPro \\
			\hline
Alcatraz Courtyard & $ 133 $ & $ 23674 $ & $\mathbf{0.52}$ & $\mathbf{0.52}$ & $ 0.57 $ & $\mathbf{0.52}$\\
Alcatraz Water Tower & $ 172 $ & $ 14828 $ & $\mathbf{0.47}$ & $ 0.63 $ & $ 0.59 $ & $\mathbf{0.47}$\\
Alcatraz West Side Gardens & $ 419 $ & $ 65072 $ & $\mathbf{0.76}$ & $ 326.99 $ & $ 1.77 $ & -\\
Basilica Di San Petronio & $ 334 $ & $ 46035 $ & $ 0.96 $ & $ 60.69 $ & $\mathbf{0.63}$ & -\\
Buddah Statue & $ 322 $ & $ 156356 $ & $ 2.93 $ & $ 96.96 $ & $\mathbf{0.41}$ & -\\
Buddah Tooth Relic Temple Singapore & $ 162 $ & $ 27920 $ & $\mathbf{0.6}$ & $ 0.62 $ & $ 0.71 $ & $\mathbf{0.6}$\\
Corridor & $ 11 $ & $ 737 $ & $\mathbf{0.26}$ & $\mathbf{0.26}$ & $ 0.27 $ & $\mathbf{0.26}$\\
Ecole Superior De Guerre & $ 35 $ & $ 13477 $ & $\mathbf{0.26}$ & $\mathbf{0.26}$ & $ 0.28 $ & $\mathbf{0.26}$\\
Dinosaur 319 & $ 36 $ & $ 319 $ & $ 1.53 $ & $\mathbf{0.43}$ & $ 0.47 $ & $\mathbf{0.43}$\\
Dinosaur 4983 & $ 36 $ & $ 4983 $ & $ 0.57 $ & $\mathbf{0.42}$ & $ 0.47 $ & $\mathbf{0.42}$\\
Doge Palace Venice & $ 241 $ & $ 67107 $ & $\mathbf{0.6}$ & $ 3.52 $ & $ 0.67 $ & -\\
Eglise du dome & $ 85 $ & $ 84792 $ & $\mathbf{0.24}$ & $\mathbf{0.24}$ & $ 0.25 $ & -\\
Drinking Fountain Somewhere in Zurich & $ 14 $ & $ 5302 $ & $\mathbf{0.28}$ & $\mathbf{0.28}$ & $ 0.31 $ & $\mathbf{0.28}$\\
East Indiaman Goteborg & $ 179 $ & $ 25655 $ & $ 0.99 $ & $ 5.11 $ & $\mathbf{0.67}$ & -\\
Folke Filbyter & $ 40 $ & $ 21150 $ & $ 8.58 $ & $ 0.82 $ & $\mathbf{0.33}$ & $ 277.89 $\\
Golden Statue Somewhere In Hong Kong & $ 18 $ & $ 39989 $ & $\mathbf{0.22}$ & $\mathbf{0.22}$ & $ 0.24 $ & $\mathbf{0.22}$\\
Gustav Vasa & $ 18 $ & $ 4249 $ & $\mathbf{0.16}$ & $\mathbf{0.16}$ & $ 0.17 $ & $\mathbf{0.16}$\\
GustavIIAdolf & $ 57 $ & $ 5813 $ & $ 5.83 $ & $\mathbf{0.23}$ & $ 0.24 $ & $\mathbf{0.23}$\\
Model House & $ 10 $ & $ 672 $ & $\mathbf{0.34}$ & $ 1.12 $ & $ 0.4 $ & $\mathbf{0.34}$\\
Jonas Ahlstromer & $ 40 $ & $ 2021 $ & $ 4.72 $ & $\mathbf{0.18}$ & $ 0.2 $ & $\mathbf{0.18}$\\
Lund University Sphinx & $ 70 $ & $ 32668 $ & $\mathbf{0.34}$ & $ 0.45 $ & $ 0.37 $ & $\mathbf{0.34}$\\
Nijo Castle Gate & $ 19 $ & $ 7348 $ & $\mathbf{0.39}$ & $\mathbf{0.39}$ & $ 0.43 $ & $\mathbf{0.39}$\\
Pantheon Paris & $ 179 $ & $ 29383 $ & $\mathbf{0.49}$ & $ 2.85 $ & $ 0.62 $ & -\\
Park Gate Clermont Ferrand & $ 34 $ & $ 9099 $ & $\mathbf{0.31}$ & $ 0.32 $ & $ 0.49 $ & $\mathbf{0.31}$\\
Plaza De Armas Santiago & $ 240 $ & $ 26969 $ & $\mathbf{0.64}$ & $ 3.14 $ & $ 0.71 $ & -\\
Porta San Donato Bologna & $ 141 $ & $ 25490 $ & $\mathbf{0.4}$ & $ 0.61 $ & $ 3.75 $ & $\mathbf{0.4}$\\
The Pumpkin & $ 195 $ & $ 69335 $ & $\mathbf{0.38}$ & $\mathbf{0.38}$ & $ 0.42 $ & -\\
Skansen Kronan Gothenburg & $ 131 $ & $ 28371 $ & $\mathbf{0.41}$ & $ 0.44 $ & $ 0.44 $ & -\\
Skansen Lejonet Gothenburg & $ 368 $ & $ 74423 $ & $ 2.05 $ & $ 7.48 $ & $\mathbf{1.28}$ & -\\
Smolny Cathedral St Petersburg & $ 131 $ & $ 51115 $ & $\mathbf{0.46}$ & $\mathbf{0.46}$ & $ 0.5 $ & -\\
Some Cathedral In Barcelona & $ 177 $ & $ 30367 $ & $\mathbf{0.51}$ & $\mathbf{0.51}$ & $ 0.54 $ & -\\
Sri Mariamman Singapore & $ 222 $ & $ 56220 $ & $\mathbf{0.61}$ & $ 0.78 $ & $ 0.85 $ & -\\
Sri Thendayuthapani Singapore & $ 98 $ & $ 88849 $ & $\mathbf{0.31}$ & $ 0.56 $ & $ 0.33 $ & -\\
Sri Veeramakaliamman Singapore & $ 157 $ & $ 130013 $ & $\mathbf{0.52}$ & $ 1.78 $ & $ 0.66 $ & -\\
Thian Hook Keng Temple Singapore & $ 138 $ & $ 34288 $ & $\mathbf{0.54}$ & $ 0.55 $ & $ 0.66 $ & $\mathbf{0.54}$\\
King's College U. of Toronto & $ 77 $ & $ 7087 $ & $ 0.78 $ & $ 2.35 $ & $ 0.26 $ & $\mathbf{0.24}$\\
Tsar Nikolai I & $ 98 $ & $ 37857 $ & $ 2.43 $ & $ 0.33 $ & $ 0.31 $ & $\mathbf{0.29}$\\
Urban II & $ 96 $ & $ 22284 $ & $ 6.84 $ & $\mathbf{0.27}$ & $ 0.31 $ & $ 3.61 $\\
			\bottomrule
	\end{tabular} 
	\end{adjustbox}
	\vspace{3pt}      
    \end{tabular}
    \caption{\small Single scene results with our method against baselines in the uncalibrated setup. The table shows average reprojection error after BA. (\textit{Smaller is better.}) In a number of experiments VarPro exceeded either memory or runtime limitations. These experiments are marked by the missing entries.}
    \label{tab:Projective_Results}
\end{table}
